Securing Satellite Link Segment: A Secure-by-Component Design

The rapid evolution of communication technologies, compounded by recent geopolitical events such as the Viasat cyberattack in February 2022, has highlighted the urgent need for fast and reliable satellite missions for military and civil security operations. Consequently, this paper examines two Earth observation (EO) missions: one utilizing a single low Earth orbit (LEO) satellite and another through a network of LEO satellites, employing a secure-by-component design strategy. This approach begins by defining the scope of technical security engineering, decomposing the system into components and data flows, and enumerating attack surfaces. Then it proceeds by identifying threats to low-level components, applying secure-by-design principles, redesigning components into secure blocks in alignment with the Space Attack Research & Tactic Analysis (SPARTA) framework, and crafting shall statements to refactor the system design, with a particular focus on improving the security of the link segment.

==> src/Secure_By_Design_and_Scope.tex <==

\section{Secure-by-Component Approach}\label{sec:SBD}

We implemented the \textit{secure-by-component} approach in \cite{Viswanathan2024} and shown in Figure \ref{figure:methodology} to obtain secure blocks. In line with the strategy, we consider SPARTA \cite{aerospace2023sparta} in listing attack techniques and secure-by-design principles.

As a first step, we define our technical scope, which encompasses the \textit{link capabilities} required for ground-to-space, space-to-ground, and, in the case of EO, space-to-space communications. 



==> tables/attack_surface_network_leo.tex <==
\begin{table}[tp]
    \caption{Attack surfaces engineering scope for mothership OBC trust.}
    \renewcommand{\arraystretch}{1.25} 
        \centering
             \scalebox{0.9}{
    \begin{tabular}{|p{2.4cm}|p{0.43cm}|p{1.25cm}|p{0.7cm}|p{2.3cm}|}
        \hline
        Component & Input & Processing & Output & Related Data Flow \\ \hline\hline
        Orbit determination & \multirow{5}{*}{\begin{turn}{90}\begin{minipage}{2.5cm}Signal from payload\\ control\end{minipage}\end{turn}} & Commands & \multirow{5}{*}{\begin{turn}{90}\begin{minipage}{2.5cm}Acknowledgement\end{minipage}\end{turn}}& Sectoring and altitude  \\ \hhline{-~-~-}
        Sectoring altitude calculation &  & Commands &  & Processed images  \\ \hhline{-~-~-}
        Maneuver calculation &  & Commands &  & Processed images  \\ \hhline{-~-~-}
        Mothership image processing &  & Image data &  & Processed images  \\ \hhline{-~-~-}
        Mothership storage &  & Image data &  & Processed images  \\ \hline
    \end{tabular}}
    \label{tab:attack_surface_network_leo}
\end{table}

==> tables/attack_surface_single_leo.tex <==
\begin{table}
    \caption{Attack surfaces engineering scope for single LEO satellite.}
    \renewcommand{\arraystretch}{1.2} 
        \centering
         \scalebox{0.9}{
    \begin{tabular}{|p{1.4cm}|p{1.4cm}|p{1.4cm}|p{1.4cm}|p{1.7cm}|}
        \hline
        Component & Input & Processing & Output & Related Data Flow \\ \hline\hline
        Ground station & Processed Images & Image data & Images & Processed images  \\ \hline
        Image processing & Raw images & Image data & Acknowledge-ment & Processed images  \\ \hline
        % Ground station & \hl{Trigger} &   & Image schedule & Image schedule \\ \hline \hline
        Payload control & Image schedule & Image schedule & Camera commands & Image schedule \\ \hline
       Camera & Image schedule & Image data & Image data & Image generation  \\ \hline
        Storage & Image data & Image data & Raw images & Image generation  \\ \hline
        Image processing & Raw images & Raw images & Processed images & Processed images  \\ \hline
    \end{tabular}}
    \label{tab:attack_surface_single_leo}
\end{table}

